Formation of Extremely Low-Mass White Dwarfs in Wide Orbits

Helium white dwarfs (WDs) with masses less than 0.3 $\rm M_{\sun}$ are known as extremely low-mass WDs (ELM WDs), which cannot be produced by single stellar evolution in theory. Generally, these stars are believed to form through binary interactions. Recently, two ELM WDs in unusually wide orbits were reported, i.e., KIC 8145411 and HE 0430-2457. Their orbital separations are too wide to be produced by the binary evolution scenario. In this work, we study the formation of wide-orbit ELM WD binaries from hierarchical triple systems. In this scenario, an ELM WD is formed from the inner binary and subsequently forms a wide binary system with the third object. We find that the merger of an evolved star with a brown dwarf in the inner binary fails to produce single ELM WDs, but Type Ia supernovae (SNe Ia) explosions can successfully do so. Furthermore, we investigate the impact of the supernova explosion on the orbital distribution of the surviving binary and find that this channel may have a probability of reproducing the orbital parameters of HE 0430-2457, but fails to reproduce the observed features of KIC 8145411. This supports recent observational recalibrations suggesting that KIC 8145411 resides in a triple system rather than a binary.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

